Introduction to the Tezos Blockchain

Tezos is an innovative blockchain that improves on several aspects compared to more established blockchains. It offers an original proof-of-stake consensus algorithm and can be used as a decentralized smart contract platform. It has the capacity to amend its own economic protocol through a voting mechanism and focuses on formal methods to improve safety.

==> oracle <==
parameter (or (timestamp :lookup_key)
              (pair
                 (timestamp :lookup_key)
                 (nat :rain_level)));
storage   ( pair
             (big_map
                (timestamp :lookup_key)
                (nat :rain_level))
             (address :oracle_manager) ) ;

code {
 UNPAIR;
 # parameter:(map,oracle_addr)
 IF_RIGHT { # feeding the oracle with data
 # (timestamp,level):(map,oracle_addr)
 # checking the data supplier is the oracle
  DIP {
    UNPAIR;SWAP;DUP;SENDER ;
      # sender:oracle_addr:oracle_addr:map
      ASSERT_CMPEQ; SWAP
      # map:oracle_addr
    };
    # (timestamp,level):map:oracle_addr
    UNPAIR; DIP{SOME};UPDATE;
    # map:oracle_addr
    PAIR ; NIL operation ; PAIR
  }
  # querying the oracle
  {
    # Getting the data
    DIP{DUP;CAR};GET;
    # (Some level|None):(map,oracle_addr)
    LEFT unit;
    # (Left (Some level|None)):(map,oracle_addr)
    # preparing the reply to the caller
    DIP {
      SENDER;
      CONTRACT (or
                  (option(nat :rain_level))
                  (unit));
      ASSERT_SOME;
      PUSH mutez 0
        };
    # param:0:sender_ctrct:(map,oracle_addr)
    TRANSFER_TOKENS ;
    NIL operation; SWAP;CONS;PAIR
  }
};

# invariant:
# - if parameter is left,
#   transfert_token (callback,data) 0 source /\ new_balance >= old_balance
#   || fail
# - iff SENDER is oracle, parameter left/left,  then map updated
# - iff SENDER is oracle, parameter left/right,  then balance retrieved

# - balance retrievable by oracle

